Context-dependent time-series prediction via HyperReservoirs

Time series prediction is a common application of reservoir computing. When the training and testing time series data contains multiple dynamical regimes, because an underlying parameter is changing, or the data in fact consists of multiple distinct systems, simple application of the reservoir computing principle produces high prediction errors. Here, we propose a HyperReservoir as an extended model of reservoir computing especially designed for such cases. The HyperReservoir combines a main reservoir with a smaller context reservoir, where the latter modulates the output weights of the former. This structure resembles the hypernetworks from deep neural network literature. However, in contrast, HyperReservoirs retain the simple training via linear regression of standard reservoir computing. We compare the proposed architecture with a conventional ESN, in which context acts at the input, and a full-matrix Conceptor, in which context modulates the reservoir state space. We evaluate all three models on time-series prediction tasks based on Lorenz and R\"ossler systems, including for varying bifurcation parameters and time sampling scales. We find that the HyperReservoir achieves the lowest mean test error in all three tasks, and particularly outperforms conceptors on data that is sampled from the same attractor but at different time scales.

==> results_numbers.tex <==
% ============================================================
% results_numbers.tex
% ============================================================
%
% IMPORTANT:
% - Numerical values in the manuscript should be referenced
%   through the macros defined here whenever possible.
% - Values below are computed from the CURRENT stored results
%   in:
%
%   results/esn_conceptor_hyper_v2/
%   results/esn_hyper_ablation_M5/
%
% - Main model selection:
%     Hyper-ESN:
%       M selected by mean validation cNMSE across seeds 0,1,2.
%     Conceptor:
%       aperture selected by mean validation cNMSE across
%       seeds 0,1,2.
%
% - Test summaries:
%       arithmetic mean +/- sample standard deviation (n=3).
%
% - Step 1 currently uses pattern-specific standardization.
%   If Step 1 is rerun with shared normalization, replace the
%   entire Step 1 block below.
%
% - Do NOT add wrong-context or Conceptor-similarity numbers
%   here until the final plotting/selection rules have been
%   aligned.
% ============================================================


% ============================================================
% GLOBAL EXPERIMENTAL CONSTANTS
% ============================================================

\newcommand{\NumModelSeeds}{\ensuremath{3}}
\newcommand{\TotalStateBudget}{\ensuremath{120}}

\newcommand{\SelectedHyperM}{\ensuremath{5}}
\newcommand{\SelectedHyperN}{\ensuremath{115}}

\newcommand{\NumTrainTrajectories}{\ensuremath{256}}
\newcommand{\NumValTrajectories}{\ensuremath{64}}
\newcommand{\NumTestTrajectories}{\ensuremath{64}}

\newcommand{\TrajectoryLength}{\ensuremath{1000}}
\newcommand{\PredictionHorizon}{\ensuremath{1}}
\newcommand{\WashoutLength}{\ensuremath{20}}

\newcommand{\RidgeAlpha}{\ensuremath{10^{-4}}}

\newcommand{\SlowTemporalScale}{\ensuremath{0.5}}
\newcommand{\FastTemporalScale}{\ensuremath{1.5}}


% ============================================================
% VALIDATION-SELECTED ARCHITECTURES
% ============================================================

% Hyper-ESN:
% Current stored results select M=5 (N=115) in all three tasks.

\newcommand{\StepOneHyperM}{\ensuremath{5}}
\newcommand{\StepOneHyperN}{\ensuremath{115}}

\newcommand{\StepTwoHyperM}{\ensuremath{5}}
\newcommand{\StepTwoHyperN}{\ensuremath{115}}

\newcommand{\StepThreeHyperM}{\ensuremath{5}}
\newcommand{\StepThreeHyperN}{\ensuremath{115}}


% Full-matrix Conceptor aperture:
% selected by mean validation cNMSE across seeds.

\newcommand{\StepOneConceptorAperture}{\ensuremath{3}}
\newcommand{\StepTwoConceptorAperture}{\ensuremath{1}}
\newcommand{\StepThreeConceptorAperture}{\ensuremath{1}}


% ============================================================
% STEP 1
% Lorenz--Rossler
%
% NOTE:
% These values correspond to the CURRENT implementation with
% pattern-specific standardization.
% Replace this whole block if Step 1 is rerun using a single
% normalization shared across Lorenz and Rossler.
% ============================================================

% ----- ESN -----

\newcommand{\StepOneESNSeedZero}{
    \ensuremath{5.566\times 10^{-2}}
}
\newcommand{\StepOneESNSeedOne}{
    \ensuremath{5.594\times 10^{-2}}
}
\newcommand{\StepOneESNSeedTwo}{
    \ensuremath{5.735\times 10^{-2}}
}

\newcommand{\StepOneESNMean}{
    \ensuremath{5.632\times 10^{-2}}
}
\newcommand{\StepOneESNSD}{
    \ensuremath{9.076\times 10^{-4}}
}


% ----- Full Conceptor, aperture = 3 -----

\newcommand{\StepOneConceptorSeedZero}{
    \ensuremath{3.464\times 10^{-2}}
}
\newcommand{\StepOneConceptorSeedOne}{
    \ensuremath{4.010\times 10^{-2}}
}
\newcommand{\StepOneConceptorSeedTwo}{
    \ensuremath{4.801\times 10^{-2}}
}

\newcommand{\StepOneConceptorMean}{
    \ensuremath{4.092\times 10^{-2}}
}
\newcommand{\StepOneConceptorSD}{
    \ensuremath{6.722\times 10^{-3}}
}


% ----- Augmented Hyper-ESN, N=115, M=5 -----

\newcommand{\StepOneHyperSeedZero}{
    \ensuremath{4.369\times 10^{-2}}
}
\newcommand{\StepOneHyperSeedOne}{
    \ensuremath{4.305\times 10^{-2}}
}
\newcommand{\StepOneHyperSeedTwo}{
    \ensuremath{4.539\times 10^{-2}}
}

\newcommand{\StepOneHyperMean}{
    \ensuremath{4.405\times 10^{-2}}
}
\newcommand{\StepOneHyperSD}{
    \ensuremath{1.210\times 10^{-3}}
}


% ----- Derived comparisons -----

% Relative reduction in mean cNMSE:
% 100 * (1 - Hyper / ESN)

\newcommand{\StepOneHyperReductionVsESN}{
    \ensuremath{21.8\%}
}

% ESN mean cNMSE divided by Hyper mean cNMSE

\newcommand{\StepOneESNOverHyper}{
    \ensuremath{1.28}
}

% Conceptor relative reduction compared with ESN

\newcommand{\StepOneConceptorReductionVsESN}{
    \ensuremath{27.3\%}
}


% ============================================================
% STEP 2
% Related Rossler regimes: c_R = 3.5 and 5.7
% ============================================================

% ----- ESN -----

\newcommand{\StepTwoESNSeedZero}{
    \ensuremath{4.659\times 10^{-4}}
}
\newcommand{\StepTwoESNSeedOne}{
    \ensuremath{5.795\times 10^{-4}}
}
\newcommand{\StepTwoESNSeedTwo}{
    \ensuremath{3.470\times 10^{-4}}
}

\newcommand{\StepTwoESNMean}{
    \ensuremath{4.641\times 10^{-4}}
}
\newcommand{\StepTwoESNSD}{
    \ensuremath{1.163\times 10^{-4}}
}


% ----- Full Conceptor, aperture = 1 -----

\newcommand{\StepTwoConceptorSeedZero}{
    \ensuremath{4.152\times 10^{-3}}
}
\newcommand{\StepTwoConceptorSeedOne}{
    \ensuremath{3.567\times 10^{-3}}
}
\newcommand{\StepTwoConceptorSeedTwo}{
    \ensuremath{8.526\times 10^{-3}}
}

\newcommand{\StepTwoConceptorMean}{
    \ensuremath{5.415\times 10^{-3}}
}
\newcommand{\StepTwoConceptorSD}{
    \ensuremath{2.710\times 10^{-3}}
}


% ----- Augmented Hyper-ESN, N=115, M=5 -----

\newcommand{\StepTwoHyperSeedZero}{
    \ensuremath{8.767\times 10^{-5}}
}
\newcommand{\StepTwoHyperSeedOne}{
    \ensuremath{7.333\times 10^{-5}}
}
\newcommand{\StepTwoHyperSeedTwo}{
    \ensuremath{7.541\times 10^{-5}}
}

\newcommand{\StepTwoHyperMean}{
    \ensuremath{7.880\times 10^{-5}}
}
\newcommand{\StepTwoHyperSD}{
    \ensuremath{7.746\times 10^{-6}}
}


% ----- Derived comparisons -----

\newcommand{\StepTwoHyperReductionVsESN}{
    \ensuremath{83.0\%}
}

\newcommand{\StepTwoESNOverHyper}{
    \ensuremath{5.89}
}

\newcommand{\StepTwoHyperReductionVsConceptor}{
    \ensuremath{98.5\%}
}

\newcommand{\StepTwoConceptorOverHyper}{
    \ensuremath{68.7}
}


% ============================================================
% STEP 3
% Same Rossler attractor under temporal scales 0.5 and 1.5
% ============================================================

% ----- ESN -----

\newcommand{\StepThreeESNSeedZero}{
    \ensuremath{4.936\times 10^{-3}}
}
\newcommand{\StepThreeESNSeedOne}{
    \ensuremath{5.401\times 10^{-3}}
}
\newcommand{\StepThreeESNSeedTwo}{
    \ensuremath{3.890\times 10^{-3}}
}

\newcommand{\StepThreeESNMean}{
    \ensuremath{4.742\times 10^{-3}}
}
\newcommand{\StepThreeESNSD}{
    \ensuremath{7.739\times 10^{-4}}
}


% ----- Full Conceptor, aperture = 1 -----

\newcommand{\StepThreeConceptorSeedZero}{
    \ensuremath{6.733\times 10^{-3}}
}
\newcommand{\StepThreeConceptorSeedOne}{
    \ensuremath{7.626\times 10^{-3}}
}
\newcommand{\StepThreeConceptorSeedTwo}{
    \ensuremath{1.794\times 10^{-2}}
}

\newcommand{\StepThreeConceptorMean}{
    \ensuremath{1.076\times 10^{-2}}
}
\newcommand{\StepThreeConceptorSD}{
    \ensuremath{6.226\times 10^{-3}}
}


% ----- Augmented Hyper-ESN, N=115, M=5 -----

\newcommand{\StepThreeHyperSeedZero}{
    \ensuremath{6.635\times 10^{-4}}
}
\newcommand{\StepThreeHyperSeedOne}{
    \ensuremath{5.315\times 10^{-4}}
}
\newcommand{\StepThreeHyperSeedTwo}{
    \ensuremath{7.376\times 10^{-4}}
}

\newcommand{\StepThreeHyperMean}{
    \ensuremath{6.442\times 10^{-4}}
}
\newcommand{\StepThreeHyperSD}{
    \ensuremath{1.044\times 10^{-4}}
}


% ----- Derived comparisons -----

\newcommand{\StepThreeHyperReductionVsESN}{
    \ensuremath{86.4\%}
}

\newcommand{\StepThreeESNOverHyper}{
    \ensuremath{7.36}
}

\newcommand{\StepThreeHyperReductionVsConceptor}{
    \ensuremath{94.0\%}
}

\newcommand{\StepThreeConceptorOverHyper}{
    \ensuremath{16.7}
}


% ============================================================
% HYPER-ESN CONTEXT-DIMENSION SWEEP
%
% Values below are TEST cNMSE mean +/- sample SD.
% Architecture selection itself is based on VALIDATION cNMSE.
% ============================================================


% ------------------------------------------------------------
% Step 1
% ------------------------------------------------------------

\newcommand{\StepOneHyperMTwoMean}{
    \ensuremath{4.885\times 10^{-2}}
}
\newcommand{\StepOneHyperMTwoSD}{
    \ensuremath{1.791\times 10^{-3}}
}

\newcommand{\StepOneHyperMFiveMean}{
    \ensuremath{4.405\times 10^{-2}}
}
\newcommand{\StepOneHyperMFiveSD}{
    \ensuremath{1.210\times 10^{-3}}
}

\newcommand{\StepOneHyperMTenMean}{
    \ensuremath{4.442\times 10^{-2}}
}
\newcommand{\StepOneHyperMTenSD}{
    \ensuremath{3.634\times 10^{-3}}
}

\newcommand{\StepOneHyperMTwentyMean}{
    \ensuremath{4.435\times 10^{-2}}
}
\newcommand{\StepOneHyperMTwentySD}{
    \ensuremath{3.070\times 10^{-3}}
}

\newcommand{\StepOneHyperMFortyMean}{
    \ensuremath{4.696\times 10^{-2}}
}
\newcommand{\StepOneHyperMFortySD}{
    \ensuremath{2.815\times 10^{-3}}
}


% ------------------------------------------------------------
% Step 2
% ------------------------------------------------------------

\newcommand{\StepTwoHyperMTwoMean}{
    \ensuremath{1.880\times 10^{-4}}
}
\newcommand{\StepTwoHyperMTwoSD}{
    \ensuremath{3.013\times 10^{-5}}
}

\newcommand{\StepTwoHyperMFiveMean}{
    \ensuremath{7.880\times 10^{-5}}
}
\newcommand{\StepTwoHyperMFiveSD}{
    \ensuremath{7.746\times 10^{-6}}
}

\newcommand{\StepTwoHyperMTenMean}{
    \ensuremath{1.104\times 10^{-4}}
}
\newcommand{\StepTwoHyperMTenSD}{
    \ensuremath{1.318\times 10^{-5}}
}

\newcommand{\StepTwoHyperMTwentyMean}{
    \ensuremath{1.424\times 10^{-4}}
}
\newcommand{\StepTwoHyperMTwentySD}{
    \ensuremath{1.530\times 10^{-5}}
}

\newcommand{\StepTwoHyperMFortyMean}{
    \ensuremath{2.557\times 10^{-4}}
}
\newcommand{\StepTwoHyperMFortySD}{
    \ensuremath{1.205\times 10^{-4}}
}


% ------------------------------------------------------------
% Step 3
% ------------------------------------------------------------

\newcommand{\StepThreeHyperMTwoMean}{
    \ensuremath{1.616\times 10^{-3}}
}
\newcommand{\StepThreeHyperMTwoSD}{
    \ensuremath{8.627\times 10^{-4}}
}

\newcommand{\StepThreeHyperMFiveMean}{
    \ensuremath{6.442\times 10^{-4}}
}
\newcommand{\StepThreeHyperMFiveSD}{
    \ensuremath{1.044\times 10^{-4}}
}

\newcommand{\StepThreeHyperMTenMean}{
    \ensuremath{6.643\times 10^{-4}}
}
\newcommand{\StepThreeHyperMTenSD}{
    \ensuremath{1.408\times 10^{-4}}
}

\newcommand{\StepThreeHyperMTwentyMean}{
    \ensuremath{8.435\times 10^{-4}}
}
\newcommand{\StepThreeHyperMTwentySD}{
    \ensuremath{3.862\times 10^{-4}}
}

\newcommand{\StepThreeHyperMFortyMean}{
    \ensuremath{7.725\times 10^{-4}}
}
\newcommand{\StepThreeHyperMFortySD}{
    \ensuremath{1.599\times 10^{-4}}
}


% ============================================================
% READOUT ABLATION AT N=115, M=5
%
% Existing stored runs:
%   - additive concatenation
%   - strict multiplicative readout
%   - augmented affine multiplicative readout
%
% Augmented values are the same M=5 results used above.
% ============================================================


% ------------------------------------------------------------
% Step 1
% ------------------------------------------------------------

\newcommand{\StepOneConcatMean}{
    \ensuremath{5.249\times 10^{-2}}
}
\newcommand{\StepOneConcatSD}{
    \ensuremath{1.024\times 10^{-3}}
}

\newcommand{\StepOneStrictMean}{
    \ensuremath{6.467\times 10^{-2}}
}
\newcommand{\StepOneStrictSD}{
    \ensuremath{7.346\times 10^{-3}}
}

\newcommand{\StepOneAugmentedMean}{
    \StepOneHyperMean
}
\newcommand{\StepOneAugmentedSD}{
    \StepOneHyperSD
}


% ------------------------------------------------------------
% Step 2
% ------------------------------------------------------------

\newcommand{\StepTwoConcatMean}{
    \ensuremath{2.071\times 10^{-4}}
}
\newcommand{\StepTwoConcatSD}{
    \ensuremath{3.444\times 10^{-5}}
}

\newcommand{\StepTwoStrictMean}{
    \ensuremath{9.101\times 10^{-2}}
}
\newcommand{\StepTwoStrictSD}{
    \ensuremath{2.202\times 10^{-2}}
}

\newcommand{\StepTwoAugmentedMean}{
    \StepTwoHyperMean
}
\newcommand{\StepTwoAugmentedSD}{
    \StepTwoHyperSD
}


% ------------------------------------------------------------
% Step 3
% ------------------------------------------------------------

\newcommand{\StepThreeConcatMean}{
    \ensuremath{2.080\times 10^{-3}}
}
\newcommand{\StepThreeConcatSD}{
    \ensuremath{1.217\times 10^{-4}}
}

\newcommand{\StepThreeStrictMean}{
    \ensuremath{1.978\times 10^{-3}}
}
\newcommand{\StepThreeStrictSD}{
    \ensuremath{9.186\times 10^{-4}}
}

\newcommand{\StepThreeAugmentedMean}{
    \StepThreeHyperMean
}
\newcommand{\StepThreeAugmentedSD}{
    \StepThreeHyperSD
}


% ============================================================
% DERIVED READOUT-ABLATION COMPARISONS
% ============================================================

% Augmented reduction relative to additive concatenation

\newcommand{\StepOneAugmentedReductionVsConcat}{
    \ensuremath{16.1\%}
}
\newcommand{\StepTwoAugmentedReductionVsConcat}{
    \ensuremath{61.9\%}
}
\newcommand{\StepThreeAugmentedReductionVsConcat}{
    \ensuremath{69.0\%}
}


% ============================================================
% READOUT FEATURE DIMENSIONS AND FITTED COEFFICIENT COUNTS
%
% Output dimension D_out = 3.
% Bias is included as one additional fitted feature.
% ============================================================

% Conventional ESN:
% feature dimension = 120
% fitted output coefficients = 3 * (120 + 1) = 363

\newcommand{\ESNReadoutFeatureDim}{
    \ensuremath{120}
}
\newcommand{\ESNReadoutNumParameters}{
    \ensuremath{363}
}


% Conceptor shared readout:
% feature dimension = 120
% fitted output coefficients = 363

\newcommand{\ConceptorReadoutFeatureDim}{
    \ensuremath{120}
}
\newcommand{\ConceptorReadoutNumParameters}{
    \ensuremath{363}
}


% M=5, N=115 Hyper-ESN
%
% Concat:
% N + M = 120
%
% Strict:
% N*M = 575
%
% Augmented:
% N + M + N*M = 695

\newcommand{\ConcatReadoutFeatureDim}{
    \ensuremath{120}
}
\newcommand{\ConcatReadoutNumParameters}{
    \ensuremath{363}
}

\newcommand{\StrictReadoutFeatureDim}{
    \ensuremath{575}
}
\newcommand{\StrictReadoutNumParameters}{
    \ensuremath{1728}
}

\newcommand{\AugmentedReadoutFeatureDim}{
    \ensuremath{695}
}
\newcommand{\AugmentedReadoutNumParameters}{
    \ensuremath{2088}
}


% Full-Conceptor context-specific matrix storage for K=2:
%
% 2 * 120 * 120 = 28,800 scalar entries.
%
% This is STORAGE, not the fitted linear-readout parameter count.

\newcommand{\ConceptorMatrixStorageKTwo}{
    \ensuremath{28\,800}
}

% If one wants to quote dense Conceptor storage plus the shared
% output readout:
%
% 28,800 + 363 = 29,163

\newcommand{\ConceptorPlusReadoutStorageKTwo}{
    \ensuremath{29\,163}
}


% ============================================================
% NUMBERS INTENTIONALLY NOT INCLUDED YET
% ============================================================
%
% 1. Wrong-context intervention:
%    Do not freeze manuscript macros until the final plotting
%    pipeline and selected architectures have been confirmed.
%
% 2. Conceptor similarity:
%    Do not freeze values until the plot uses the SAME
%    task-level validation-selected aperture as the main
%    comparison.
%
% 3. Any Step 1 result after removal of pattern-specific
%    standardization:
%    No such rerun has yet been performed.
%
% ============================================================
